Bayesian Algorithms for Kronecker-structured Sparse Vector Recovery With Application to IRS-MIMO Channel Estimation

We study the sparse recovery problem with an underdetermined linear system characterized by a Kronecker-structured dictionary and a Kronecker-supported sparse vector. We cast this problem into the sparse Bayesian learning (SBL) framework and rely on the expectation-maximization method for a solution. To this end, we model the Kronecker-structured support with a hierarchical Gaussian prior distribution parameterized by a Kronecker-structured hyperparameter, leading to a non-convex optimization problem. The optimization problem is solved using the alternating minimization (AM) method and a singular value decomposition (SVD)-based method, resulting in two algorithms. Further, we analytically guarantee that the AM-based method converges to the stationary point of the SBL cost function. The SVD-based method, though it adopts approximations, is empirically shown to be more efficient and accurate. We then apply our algorithm to estimate the uplink wireless channel in an intelligent reflecting surface-aided MIMO system and extend the AM-based algorithm to address block sparsity in the channel. We also study the SBL cost to show that the minima of the cost function are achieved at sparse solutions and that incorporating the Kronecker structure reduces the number of local minima of the SBL cost function. Our numerical results demonstrate the effectiveness of our algorithms compared to the state-of-the-art.

==> basestation.tex <==

% chktex-file 1
% chktex-file 27

\makeatletter


% The keys that the user can provide are all the keys below.

% Keys for the Beam shape
\pgfkeys{
  /pgf/.cd,
  % The 4 following options control the proportion of shapewidth/shapeheight for
  % the control points of the beam -> The must be greater than zero
  control point 1 x/.initial=0.35,
  control point 1 y/.initial=1.0,
  control point 2 x/.initial=0.5,
  control point 2 y/.initial=0.25,
}

% Keys for the UserTerminal shape
\pgfkeys{
  /pgf/.cd,
  button fill color/.initial=white,
  screen fill color/.initial=white,
}


% Represents a "beam", which is constructed using two Bézier curves.
% The two control points can be controlled by passing the
% "control point 1 x/control point 1 y/control point 2 x/control point 2 y"
% parameters.
\pgfdeclareshape{Beam}{

  % xxxxxxxxxx Define some saved macros xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  \savedmacro\shapewidth{
    \def\shapewidth{\pgfkeysvalueof{/pgf/minimum width}}
  }

  \savedmacro\shapeheight{
    \def\shapeheight{\pgfkeysvalueof{/pgf/minimum height}}
  }

  \savedmacro\firstpointxprop{
    \def\firstpointxprop{\pgfkeysvalueof{/pgf/control point 1 x}}
  }
  \savedmacro\firstpointyprop{
    \def\firstpointyprop{\pgfkeysvalueof{/pgf/control point 1 y}}
  }
  \savedmacro\secondpointxprop{
    \def\secondpointxprop{\pgfkeysvalueof{/pgf/control point 2 x}}
  }
  \savedmacro\secondpointyprop{
    \def\secondpointyprop{\pgfkeysvalueof{/pgf/control point 2 y}}
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  \savedanchor\startpoint{%
    \pgfmathsetlength\pgf@x{-0.5*\shapewidth}
    \pgfmathsetlength\pgf@y{0}
  }

  \savedanchor\endpoint{%
    \pgfmathsetlength\pgf@x{0.5*\shapewidth}
    \pgfmathsetlength\pgf@y{0}
  }

  % \savedanchor\centerpoint{%
  %   \pgf@x=0%
  %   \pgf@y=0%
  % }

  % Control point anchors
  \savedanchor\firstcontrolpointtop{%
    \pgfmathsetlength\pgf@x{\firstpointxprop*\shapewidth}
    \pgfmathsetlength\pgf@y{\firstpointyprop*\shapeheight}
  }

  \savedanchor\secondcontrolpointtop{%
    \pgfmathsetlength\pgf@x{\secondpointxprop*\shapewidth}
    \pgfmathsetlength\pgf@y{\secondpointyprop*\shapeheight}
  }

  \savedanchor\firstcontrolpointbottom{%
    \pgfmathsetlength\pgf@x{\firstpointxprop*\shapewidth}
    \pgfmathsetlength\pgf@y{-\firstpointyprop*\shapeheight}
  }

  \savedanchor\secondcontrolpointbottom{%
    \pgfmathsetlength\pgf@x{\secondpointxprop*\shapewidth}
    \pgfmathsetlength\pgf@y{-\secondpointyprop*\shapeheight}
  }

  % xxxxxxxxxx Define regular anchors xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  \anchor{center}{\startpoint}
  \anchor{start}{\startpoint}
  \anchor{end}{\endpoint}
  \anchor{main region}{
    \endpoint
    \pgfmathsetlength\pgf@x{\pgf@x-0.25*\shapewidth}
  }
  \anchor{top control point 1}{\firstcontrolpointtop}
  \anchor{top control point 2}{\secondcontrolpointtop}
  \anchor{bottom control point 1}{\firstcontrolpointbottom}
  \anchor{bottom control point 2}{\secondcontrolpointbottom}
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  \inheritanchorborder[from=rectangle]

  % xxxxxxxxxx Draw the background path xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  \backgroundpath{
    \begin{pgfscope}
      \pgfmoveto{\startpoint}
      \pgfcurveto{\firstcontrolpointtop}{\secondcontrolpointtop}{\endpoint}
      \pgfcurveto{\secondcontrolpointbottom}{\firstcontrolpointbottom}{\startpoint}
      \pgfpathclose
      \pgfusepath{stroke,fill}
    \end{pgfscope}
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
}


% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxx UserTerminal Shape xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
\pgfdeclareshape{UserTerminal}{

  % xxxxxxxxxx First we define some savedmacros xxxxxxxxxxxxxxxxxxxxxxxxxxx
  % Macros and savedanchors common to UserTerminal and BaseStation Shapes
  \savedanchor{\center}{
    \pgf@x=0pt
    \pgf@y=0pt
  }

  % Note that pgf provides the text macros \pgfshapeminwidth and
  % pgfshapeminheight that store the minim width and minimum height,
  % respectivelly. Note that They are "TEXT macros" and not
  % "lengths". Calling them simple
  % replaces for the text.
  \savedanchor{\northeast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=0.5\pgf@xa
    \pgf@y=0.5\pgf@ya
    % NOTE: We can't use 0.5\pgfshapeminwidth directly because the minimum
    % width is stored in a "plain text macro". If minimum width is 2cm, for
    % instance, and we write "\pgf@x=.5\pgfshapeminwidth" then \pgf@x would
    % be set to 0.52cm, which is not what we want. See the explanation for
    % \savedanchor in the pgfmanual (page 627).
  }

  \savedanchor{\southwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=-0.5\pgf@xa
    \pgf@y=-0.5\pgf@ya
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  % Savedanchors specific to the UserTerminal shape
  \savedanchor{\screennortheast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=0.45\pgf@xa
    \pgf@y=0.45\pgf@ya
  }

  \savedanchor{\screensouthwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=-0.45\pgf@xa
    \pgf@y=-0.35\pgf@ya
  }

  \savedanchor{\buttonsouthwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=0pt
    \pgf@y=-0.425\pgf@ya
    \advance\pgf@x by -0.15\pgf@xa
    \advance\pgf@y by -0.04\pgf@ya
  }

  \savedanchor{\buttonnortheast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=0pt
    \pgf@y=-0.425\pgf@ya
    \advance\pgf@x by 0.15\pgf@xa
    \advance\pgf@y by 0.04\pgf@ya
  }

  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit anchor border from rectangle xxxxxxxxxxxxxxxxxxxxxxx
  \inheritanchorborder[from=rectangle]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit normal anchors from rectangle xxxxxxxxxxxxxxxxxxxxxx
  % We define the savedanchors "northeast" and "southwest". With these two
  % defined we can inherit code for the regular anchors from the
  % rectangle shape (even thought the northeast and southwest saved anchors
  % in the rectangle shape are different from ours).
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{north}
  \inheritanchor[from=rectangle]{east}
  \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{west}
  \inheritanchor[from=rectangle]{north east}
  \inheritanchor[from=rectangle]{north west}
  \inheritanchor[from=rectangle]{south west}
  \inheritanchor[from=rectangle]{south east}
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Now we define more regular anchors xxxxxxxxxxxxxxxxxxxxxxxxx
  \anchor{text}
  {
    % This will get the center of the screen
    \pgfpointlineattime{0.5}{\screensouthwest}{\screennortheast}
    % Lets put the center of the text in the center of the screen
    \advance\pgf@x by -0.5\wd\pgfnodeparttextbox
    \advance\pgf@y by -0.5\ht\pgfnodeparttextbox
  }

  \anchor{button}{
    \pgfpointlineattime{0.5}{\buttonsouthwest}{\buttonnortheast}
  }

  \anchor{screen}{
    \pgfpointlineattime{0.5}{\screensouthwest}{\screennortheast}
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Draw the background xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  \backgroundpath{
    % Scope for Terminal Body
    \begin{pgfscope}
      \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
      % '\pgfshapeminheight' cannot be used directly; or if you want to use it directly use the '*' for multiplication
      \pgfsetcornersarced{\pgfpoint{0.03\pgf@ya}{0.03\pgf@ya}}
      \pgfpathrectanglecorners
      {\southwest}
      {\northeast}
      \pgfusepath{stroke,fill}
    \end{pgfscope}

    % Scope for the terminal Screen
    \begin{pgfscope}
      \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
      \pgfsetcornersarced{\pgfpoint{0.03\pgf@ya}{0.03\pgf@ya}}
      \pgfsetfillcolor{\pgfkeysvalueof{/pgf/screen fill color}}
      %\pgfsetfillcolor{white}
      \pgfpathrectanglecorners
      {\screensouthwest}
      {\screennortheast}
      \pgfusepath{stroke,fill}
    \end{pgfscope}

    % Scope for the button
    \begin{pgfscope}
      \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
      \pgfsetcornersarced{\pgfpoint{0.009\pgf@ya}{0.009\pgf@ya}}
      \pgfsetfillcolor{\pgfkeysvalueof{/pgf/button fill color}}
      %\pgfsetfillcolor{white}
      \pgfpathrectanglecorners
      {\buttonsouthwest}
      {\buttonnortheast}
      \pgfusepath{stroke,fill}
    \end{pgfscope}
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
}
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxx END xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx


% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxx BaseStationSimple xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
\pgfdeclareshape{BaseStationSimple}{

  % xxxxxxxxxx Define savedanchors xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  % Inherit all savedanchors from UserTerminal. We only need northeast and
  % southwest, but we can't choose which ones to inherit.
  \inheritsavedanchors[from=UserTerminal]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxx Define savedanchors specific to the BaseStation shape xxxxxxxxxxx
  \savedanchor{\BaseAsouthwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@y=-0.5\pgf@ya
    \pgf@x=-0.12\pgf@xa
  }

  \savedanchor{\BaseAnortheast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@y=0.30\pgf@ya
    \pgf@x=0.12\pgf@xa
  }

  % Maybe I don't need this savedanchor
  \savedanchor{\MiddleAntennasouth}{
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=0pt
    \pgf@y=0.29\pgf@ya
  }

  \savedanchor{\AntennaConnectorsouthwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=-0.5\pgf@xa
    \pgf@y=0.38\pgf@ya
  }

  \savedanchor{\AntennaConnectornortheast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=0.5\pgf@xa
    \pgf@y=0.42\pgf@ya
  }

  \savedanchor{\MiddleAntennasouthwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=-0.15\pgf@xa
    \pgf@y=0.29\pgf@ya
  }

  \savedanchor{\MiddleAntennanortheast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=0.15\pgf@xa
    \pgf@y=0.5\pgf@ya
  }

  \savedanchor{\LeftAntennasouthwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=-0.5\pgf@xa
    \pgf@y=0.29\pgf@ya
  }

  \savedanchor{\LeftAntennanortheast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=-0.25\pgf@xa
    \pgf@y=0.5\pgf@ya
  }

  \savedanchor{\RightAntennasouthwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=0.25\pgf@xa
    \pgf@y=0.29\pgf@ya
  }

  \savedanchor{\RightAntennanortheast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=0.5\pgf@xa
    \pgf@y=0.5\pgf@ya
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit anchor border from UserTerminal xxxxxxxxxxxxxxxxxxxx
  \inheritanchorborder[from=UserTerminal]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit normal anchors from UserTerminal xxxxxxxxxxxxxxxxxxx
  % We define the savedanchors "northeast" and "southwest". With these two
  % defined we can inherit code for the regular anchors from the
  % UserTerminal shape (even thought the northeast and southwest saved anchors
  % in the UserTerminal shape are different from ours).
  \inheritanchor[from=UserTerminal]{center}
  \inheritanchor[from=UserTerminal]{north}
  \inheritanchor[from=UserTerminal]{east}
  \inheritanchor[from=UserTerminal]{south}
  \inheritanchor[from=UserTerminal]{west}
  \inheritanchor[from=UserTerminal]{north east}
  \inheritanchor[from=UserTerminal]{north west}
  \inheritanchor[from=UserTerminal]{south west}
  \inheritanchor[from=UserTerminal]{south east}
  \inheritanchor[from=rectangle]{text}
  \anchor{antenna right}{
    \northeast
    \pgfmathsetlength\pgf@y{0.8*\pgf@y}
  }
  \anchor{antenna left}{
    \northeast
    \pgfmathsetlength\pgf@y{0.8*\pgf@y}
    \pgfmathsetlength\pgf@x{-\pgf@x}
  }
  \anchor{antenna center}{
    \northeast
    \pgfmathsetlength\pgf@y{0.8*\pgf@y}
    \pgfmathsetlength\pgf@x{0}
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Draw the "behind background" xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  % The base of the antenna will be in the behindbackgroundpath while the
  % antennas will be in the backgroundpath.
  \behindbackgroundpath{
    % Scope for the Base
    \begin{pgfscope}
      % Draw the bottom base
      \pgfpathrectanglecorners
      {\BaseAsouthwest}
      {\BaseAnortheast}

      \pgfusepath{stroke,fill}
    \end{pgfscope}
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Draw the background xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  % The base of the antenna will be in the behindbackgroundpath while the
  % antennas will be in the backgroundpath. The main reason for this
  % separation is that this code here will be inherited in the
  % "BaseStation" shape that we will define later.
  \backgroundpath{
    % Scope for the antenna connector
    \begin{pgfscope}
      % Draw Antenna connector
      \pgfpathrectanglecorners
      {\AntennaConnectorsouthwest}
      {\AntennaConnectornortheast}

      \pgfusepath{stroke,fill}
    \end{pgfscope}

    % Scope for the antennas
    \begin{pgfscope}
      % Draw the middle antenna
      \pgfpathrectanglecorners
      {\MiddleAntennasouthwest}
      {\MiddleAntennanortheast}

      % Draw the Left antenna
      \pgfpathrectanglecorners
      {\LeftAntennasouthwest}
      {\LeftAntennanortheast}

      % Draw the Right antenna
      \pgfpathrectanglecorners
      {\RightAntennasouthwest}
      {\RightAntennanortheast}

      \pgfusepath{stroke,fill}
    \end{pgfscope}
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
}
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxx END xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx


% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxx BaseStation Shape xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
\pgfdeclareshape{BaseStation}{

  % xxxxxxxxxx Define savedanchors xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  % Inherit all savedanchors from BaseStationSimple.
  \inheritsavedanchors[from=BaseStationSimple]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxx Define savedanchors specific to the BaseStation shape xxxxxxxxxxx
  \savedanchor{\BaseAsouthwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@y=-0.5\pgf@ya
    \pgf@x=-0.2\pgf@xa
  }

  \savedanchor{\BaseAnortheast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@y=-0.05\pgf@ya
    \pgf@x=0.2\pgf@xa
  }

  \savedanchor{\BaseBsoutheast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@y=-0.05\pgf@ya
    \pgf@x=0.15\pgf@xa
  }

  \savedanchor{\BaseBnorthwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@y=0.15\pgf@ya
    \pgf@x=-0.15\pgf@xa
  }

  \savedanchor{\BaseCsouthwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@y=0.15\pgf@ya
    \pgf@x=-0.1\pgf@xa
  }

  \savedanchor{\BaseCnortheast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@y=0.30\pgf@ya
    \pgf@x=0.1\pgf@xa
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit anchor border from BaseStationSimple xxxxxxxxxxxxxxx
  \inheritanchorborder[from=BaseStationSimple]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit normal anchors from BaseStationSimple xxxxxxxxxxxxxx
  % We define the savedanchors "northeast" and "southwest". With these two
  % defined we can inherit code for the regular anchors from the
  % BaseStationSimple shape (even thought the northeast and southwest saved anchors
  % in the BaseStationSimple shape are different from ours)..
  \inheritanchor[from=BaseStationSimple]{center}
  \inheritanchor[from=BaseStationSimple]{north}
  \inheritanchor[from=BaseStationSimple]{east}
  \inheritanchor[from=BaseStationSimple]{south}
  \inheritanchor[from=BaseStationSimple]{west}
  \inheritanchor[from=BaseStationSimple]{north east}
  \inheritanchor[from=BaseStationSimple]{north west}
  \inheritanchor[from=BaseStationSimple]{south west}
  \inheritanchor[from=BaseStationSimple]{south east}
  \inheritanchor[from=BaseStationSimple]{antenna right}
  \inheritanchor[from=BaseStationSimple]{antenna left}
  \inheritanchor[from=BaseStationSimple]{antenna center}
  \inheritanchor[from=rectangle]{text}
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Draw the "behind background" xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  \behindbackgroundpath{
    % Scope for the Base
    \begin{pgfscope}
      % Draw the bottom base
      \pgfpathrectanglecorners
      {\BaseAsouthwest}
      {\BaseAnortheast}

      % Draw the middle base
      \pgfpathrectanglecorners
      {\BaseBsoutheast}
      {\BaseBnorthwest}

      % Draw the bottom base
      \pgfpathrectanglecorners
      {\BaseCsouthwest}
      {\BaseCnortheast}

      \pgfusepath{stroke,fill}
    \end{pgfscope}
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxx Inherit the background path from BaseStationSimple xxxxxxxxxxx
  \inheritbackgroundpath[from=BaseStationSimple]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
}
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxx END xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

\makeatother

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "testbasestation.tex"
%%% TeX-PDF-mode: t
%%% End:

==> irs.tex <==
% chktex-file 1
% chktex-file 27

\makeatletter

% The keys that the user can provide are all the keys below.

\pgfkeys{
  /pgf/.cd,
  element fill color/.initial=white,
}


\pgfdeclareshape{IRS}{

  % xxxxxxxxxx Define some saved macros xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  \savedmacro\shapewidth{
    \def\shapewidth{\pgfkeysvalueof{/pgf/minimum width}}
  }

  \savedmacro\shapeheight{
    \def\shapeheight{\pgfkeysvalueof{/pgf/minimum height}}
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Saved Anchors for each element top left and bottom right xxxxxxxx
  % 
  % The IRS elements are named with single capital letters in a
  % rowwise fashion. That is, element 1-1 is A, element 1-2 is B, and
  % so on.
  % 
  % The width/height of each IRS element is 0.2 of the full IRS
  % width/height. The spacing between elements is 0.04 of the width/height.
  
  % First row
  \savedanchor\elementAtopleft{%
    \pgfmathsetlength\pgf@x{-0.46*\shapewidth}
    \pgfmathsetlength\pgf@y{0.46*\shapeheight}
  }

  \savedanchor\elementAbottomright{%
    \pgfmathsetlength\pgf@x{-0.26*\shapewidth}
    \pgfmathsetlength\pgf@y{0.26*\shapeheight}
  }
  
  \savedanchor\elementBtopleft{%
    \pgfmathsetlength\pgf@x{-0.22*\shapewidth}
    \pgfmathsetlength\pgf@y{0.46*\shapeheight}
  }

  \savedanchor\elementBbottomright{%
    \pgfmathsetlength\pgf@x{-0.02*\shapewidth}
    \pgfmathsetlength\pgf@y{0.26*\shapeheight}
  }

  \savedanchor\elementCtopleft{%
    \pgfmathsetlength\pgf@x{0.02*\shapewidth}
    \pgfmathsetlength\pgf@y{0.46*\shapeheight}
  }

  \savedanchor\elementCbottomright{%
    \pgfmathsetlength\pgf@x{0.22*\shapewidth}
    \pgfmathsetlength\pgf@y{0.26*\shapeheight}
  }

  \savedanchor\elementDtopleft{%
    \pgfmathsetlength\pgf@x{0.26*\shapewidth}
    \pgfmathsetlength\pgf@y{0.46*\shapeheight}
  }

  \savedanchor\elementDbottomright{%
    \pgfmathsetlength\pgf@x{0.46*\shapewidth}
    \pgfmathsetlength\pgf@y{0.26*\shapeheight}
  }
  
%   Cdots
  \savedanchor\elementctopleft{%
    \pgfmathsetlength\pgf@x{0.74*\shapewidth}
    \pgfmathsetlength\pgf@y{0.46*\shapeheight}
  }

  \savedanchor\elementcbottomright{%
    \pgfmathsetlength\pgf@x{0.94*\shapewidth}
    \pgfmathsetlength\pgf@y{0.26*\shapeheight}
  }

%   Second Row
  \savedanchor\elementEtopleft{%
    \pgfmathsetlength\pgf@x{0.74*\shapewidth}
    \pgfmathsetlength\pgf@y{0.46*\shapeheight}
  }

  \savedanchor\elementEbottomright{%
    \pgfmathsetlength\pgf@x{0.94*\shapewidth}
    \pgfmathsetlength\pgf@y{0.26*\shapeheight}
  }
  
%   \savedanchor\elementFtopleft{%
%     \pgfmathsetlength\pgf@x{-0.22*\shapewidth}
%     \pgfmathsetlength\pgf@y{0.22*\shapeheight}
%   }

%   \savedanchor\elementFbottomright{%
%     \pgfmathsetlength\pgf@x{-0.02*\shapewidth}
%     \pgfmathsetlength\pgf@y{0.02*\shapeheight}
%   }

%   \savedanchor\elementGtopleft{%
%     \pgfmathsetlength\pgf@x{0.02*\shapewidth}
%     \pgfmathsetlength\pgf@y{0.22*\shapeheight}
%   }

%   \savedanchor\elementGbottomright{%
%     \pgfmathsetlength\pgf@x{0.22*\shapewidth}
%     \pgfmathsetlength\pgf@y{0.02*\shapeheight}
%   }

%   \savedanchor\elementHtopleft{%
%     \pgfmathsetlength\pgf@x{0.26*\shapewidth}
%     \pgfmathsetlength\pgf@y{0.22*\shapeheight}
%   }

%   \savedanchor\elementHbottomright{%
%     \pgfmathsetlength\pgf@x{0.46*\shapewidth}
%     \pgfmathsetlength\pgf@y{0.02*\shapeheight}
%   }

%   % Third Row
%   \savedanchor\elementItopleft{%
%     \pgfmathsetlength\pgf@x{-0.46*\shapewidth}
%     \pgfmathsetlength\pgf@y{-0.02*\shapeheight}
%   }

%   \savedanchor\elementIbottomright{%
%     \pgfmathsetlength\pgf@x{-0.26*\shapewidth}
%     \pgfmathsetlength\pgf@y{-0.22*\shapeheight}
%   }
  
%   \savedanchor\elementJtopleft{%
%     \pgfmathsetlength\pgf@x{-0.22*\shapewidth}
%     \pgfmathsetlength\pgf@y{-0.02*\shapeheight}
%   }

%   \savedanchor\elementJbottomright{%
%     \pgfmathsetlength\pgf@x{-0.02*\shapewidth}
%     \pgfmathsetlength\pgf@y{-0.22*\shapeheight}
%   }

%   \savedanchor\elementKtopleft{%
%     \pgfmathsetlength\pgf@x{0.02*\shapewidth}
%     \pgfmathsetlength\pgf@y{-0.02*\shapeheight}
%   }

%   \savedanchor\elementKbottomright{%
%     \pgfmathsetlength\pgf@x{0.22*\shapewidth}
%     \pgfmathsetlength\pgf@y{-0.22*\shapeheight}
%   }

%   \savedanchor\elementLtopleft{%
%     \pgfmathsetlength\pgf@x{0.26*\shapewidth}
%     \pgfmathsetlength\pgf@y{-0.02*\shapeheight}
%   }

%   \savedanchor\elementLbottomright{%
%     \pgfmathsetlength\pgf@x{0.46*\shapewidth}
%     \pgfmathsetlength\pgf@y{-0.22*\shapeheight}
%   }

%   % Forth Row
%   \savedanchor\elementMtopleft{%
%     \pgfmathsetlength\pgf@x{-0.46*\shapewidth}
%     \pgfmathsetlength\pgf@y{-0.26*\shapeheight}
%   }

%   \savedanchor\elementMbottomright{%
%     \pgfmathsetlength\pgf@x{-0.26*\shapewidth}
%     \pgfmathsetlength\pgf@y{-0.46*\shapeheight}
%   }
  
%   \savedanchor\elementNtopleft{%
%     \pgfmathsetlength\pgf@x{-0.22*\shapewidth}
%     \pgfmathsetlength\pgf@y{-0.26*\shapeheight}
%   }

%   \savedanchor\elementNbottomright{%
%     \pgfmathsetlength\pgf@x{-0.02*\shapewidth}
%     \pgfmathsetlength\pgf@y{-0.46*\shapeheight}
%   }

%   \savedanchor\elementOtopleft{%
%     \pgfmathsetlength\pgf@x{0.02*\shapewidth}
%     \pgfmathsetlength\pgf@y{-0.26*\shapeheight}
%   }

%   \savedanchor\elementObottomright{%
%     \pgfmathsetlength\pgf@x{0.22*\shapewidth}
%     \pgfmathsetlength\pgf@y{-0.46*\shapeheight}
%   }

%   \savedanchor\elementPtopleft{%
%     \pgfmathsetlength\pgf@x{0.26*\shapewidth}
%     \pgfmathsetlength\pgf@y{-0.26*\shapeheight}
%   }

%   \savedanchor\elementPbottomright{%
%     \pgfmathsetlength\pgf@x{0.46*\shapewidth}
%     \pgfmathsetlength\pgf@y{-0.46*\shapeheight}
%   }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  
  % xxxxxxxxxx Define savedanchors xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  % Inherit all savedanchors from UserTerminal. We only need northeast and
  % southwest, but we can't choose which ones to inherit.
  \inheritsavedanchors[from=rectangle]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxx Define savedanchors specific to the BaseStation shape xxxxxxxxxxx
  % NONE
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit anchor border from UserTerminal xxxxxxxxxxxxxxxxxxxx
  \inheritanchorborder[from=rectangle]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit normal anchors from UserTerminal xxxxxxxxxxxxxxxxxxx
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{north}
  \inheritanchor[from=rectangle]{east}
  \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{west}
  \inheritanchor[from=rectangle]{north east}
  \inheritanchor[from=rectangle]{north west}
  \inheritanchor[from=rectangle]{south west}
  \inheritanchor[from=rectangle]{south east}
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  
  % xxxxxxxxxx Draw the background path xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  \backgroundpath{

    % \begin{pgfscope}
    %   % \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    %   % '\pgfshapeminheight' cannot be used directly; or if you want to use it directly use the '*' for multiplication
    %   % \pgfsetcornersarced{\pgfpoint{0.03\pgf@ya}{0.03\pgf@ya}}
    %   \pgfpathrectanglecorners
    %   {\southwest}
    %   {\northeast}
    % %   \pgfusepath{stroke,fill}
    % \end{pgfscope}

    \begin{scope} % Scope for all IRS elements to make the rounded corners
      \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
      \pgfsetcornersarced{\pgfpoint{0.03\pgf@ya}{0.03\pgf@ya}}
      \pgfsetfillcolor{\pgfkeysvalueof{/pgf/element fill color}}
      
      % IRS Element 1-1
      \begin{scope}
        \pgfpathrectanglecorners
        {\elementAtopleft}
        {\elementAbottomright}
        \pgfusepath{stroke,fill}
      \end{scope}

      % IRS Element 1-2
      \begin{scope}
        \pgfpathrectanglecorners
        {\elementBtopleft}
        {\elementBbottomright}
        \pgfusepath{stroke,fill}
      \end{scope}

      % IRS Element 1-3
      \begin{scope}
        \pgfpathrectanglecorners
        {\elementCtopleft}
        {\elementCbottomright}
        \pgfusepath{stroke,fill}
      \end{scope}

      % IRS Element 1-4
      \begin{scope}
        \pgfpathrectanglecorners
        {\elementDtopleft}
        {\elementDbottomright}
        \pgfusepath{stroke,fill}
      \end{scope}

      % IRS Element 2-1
      \begin{scope}
        \pgfpathrectanglecorners
        {\elementEtopleft}
        {\elementEbottomright}
        \pgfusepath{stroke,fill}
      \end{scope}
      
      % Cdots
    %   \node[\elementctopleft] {$\tiny\cdots$}
      
    %   % IRS Element 2-2
    %   \begin{scope}
    %     \pgfpathrectanglecorners
    %     {\elementFtopleft}
    %     {\elementFbottomright}
    %     \pgfusepath{stroke,fill}
    %   \end{scope}

    %   % IRS Element 2-3
    %   \begin{scope}
    %     \pgfpathrectanglecorners
    %     {\elementGtopleft}
    %     {\elementGbottomright}
    %     \pgfusepath{stroke,fill}
    %   \end{scope}

    %   % IRS Element 2-4
    %   \begin{scope}
    %     \pgfpathrectanglecorners
    %     {\elementHtopleft}
    %     {\elementHbottomright}
    %     \pgfusepath{stroke,fill}
    %   \end{scope}

    %   % IRS Element 3-1
    %   \begin{scope}
    %     \pgfpathrectanglecorners
    %     {\elementItopleft}
    %     {\elementIbottomright}
    %     \pgfusepath{stroke,fill}
    %   \end{scope}

    %   % IRS Element 3-2
    %   \begin{scope}
    %     \pgfpathrectanglecorners
    %     {\elementJtopleft}
    %     {\elementJbottomright}
    %     \pgfusepath{stroke,fill}
    %   \end{scope}

    %   % IRS Element 3-3
    %   \begin{scope}
    %     \pgfpathrectanglecorners
    %     {\elementKtopleft}
    %     {\elementKbottomright}
    %     \pgfusepath{stroke,fill}
    %   \end{scope}

    %   % IRS Element 3-4
    %   \begin{scope}
    %     \pgfpathrectanglecorners
    %     {\elementLtopleft}
    %     {\elementLbottomright}
    %     \pgfusepath{stroke,fill}
    %   \end{scope}

    %   % IRS Element 4-1
    %   \begin{scope}
    %     \pgfpathrectanglecorners
    %     {\elementMtopleft}
    %     {\elementMbottomright}
    %     \pgfusepath{stroke,fill}
    %   \end{scope}

    %   % IRS Element 4-2
    %   \begin{scope}
    %     \pgfpathrectanglecorners
    %     {\elementNtopleft}
    %     {\elementNbottomright}
    %     \pgfusepath{stroke,fill}
    %   \end{scope}

    %   % IRS Element 4-3
    %   \begin{scope}
    %     \pgfpathrectanglecorners
    %     {\elementOtopleft}
    %     {\elementObottomright}
    %     \pgfusepath{stroke,fill}
    %   \end{scope}

    %   % IRS Element 4-4
    %   \begin{scope}
    %     \pgfpathrectanglecorners
    %     {\elementPtopleft}
    %     {\elementPbottomright}
    %     \pgfusepath{stroke,fill}
    %   \end{scope}
    \end{scope}
    
    % \begin{pgfscope}
    %   \pgfmoveto{\startpoint}
    %   \pgfcurveto{\firstcontrolpointtop}{\secondcontrolpointtop}{\endpoint}
    %   \pgfcurveto{\secondcontrolpointbottom}{\firstcontrolpointbottom}{\startpoint}
    %   \pgfpathclose
    %   \pgfusepath{stroke,fill}
    % \end{pgfscope}
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "test_irs.tex"
%%% End:
